On Fault Tolerance of Data Storage Systems: A Holistic Perspective

Data storage systems serve as the foundation of digital society. The enormous data generated by people on a daily basis make the fault tolerance of data storage systems increasingly important. Unfortunately, modern storage systems consist of complicated hardware and software layers interacting with each other, which may contain latent bugs that elude extensive testing and lead to data corruption, system downtime, or even unrecoverable data loss in practice. In this chapter, we take a holistic view to introduce the typical architecture and major components of modern data storage systems (e.g., solid state drives, persistent memories, local file systems, and distributed storage management at scale). Next, we discuss a few representative bug detection and fault tolerance techniques across layers with a focus on issues that affect system recovery and data integrity. Finally, we conclude with open challenges and future work.

==> linuxFaultInjection.tex <==
\subsection{Fault Injection Techniques}
\subsubsection{Linux Fault Injection (LFI)} %Ahmed (status: review)
There are many fault injection tools available in both the community and academia. Still, a black-box fault injection mechanism is found in the Linux kernel starting from version 2.6.20, called Linux fault injection or (LFI). LFI is used to inject artificial faults into devices (i.e., memory and block devices) \cite{Naughton}. However, the injection feature is present in the Linux kernel source code; it is turned off by default, and activating it requires declaring specific directives in the kernel configuration and compiling it. 

It is worth noting that the injection mechanism is completely neglected if it is not enabled. After configuring the kernel for fault injection, the next step is injecting faults into the target device through the debugging file system (debugfs) \cite{LFI_doc}, considered a fault configuration at runtime. 

The fault injection is done by filling the fault capabilities directly through debugfs, where the device driver that has been designed to be injected reads those capabilities and does the injection. Linux has a predefined script (failcmd.sh) to inject the slab memory fault; the script is nothing more than a fuser-friendly bash script that utilizes the debugfs.

When the injection value is received in the target device driver, the function (should\_fail) is triggered and causes the failure. Since the injection system is at the operating system level, errors can be directed through the userspace and system level. Finally, the (dmesg) tool collects kernel messages, including the failure caused by the (should\_fail) function. Figure \ref{fig:LFI_flow} illustrates the LFI flow diagram.

Since Linux is an open-source system, it is easy to extend the injection mechanism to include new capabilities and support more devices by adding the (should\_fail) function in the device driver, as will be explained in section \ref{section:add_new_LFI}

\begin{figure}[ht!]
    %https://app.diagrams.net/#G1X0OPUgUQQkQoM-37r9kAi8EktWl2QWuQ#%7B%22pageId%22%3A%22Usf-SLBHwVmOU5nxGpp_%22%7D
    \centering
    \includegraphics[scale=0.50]{LFI/LFI_flow.png}
    \caption{Linux Fault Injection Flow diagram}
    \label{fig:LFI_flow}
\end{figure}


%https://github.com/torvalds/linux/blob/fbfd64d25c7af3b8695201ebc85efe90be28c5a3/lib/fault-inject.c#L401
The fault injection framework implementation is located in the Linux source code under the path (lib/fault-inject.c). The implementation is straightforward. It reads the input (e.g., interval, probability, etc.) from the debugfs string and stores the result in the fault attribute structure (fault\_attr). The core function is "should\_fail\_ex", which examines the capabilities, returns true if they are met, indicating a failure, or returns false if not.

\subsubsection{Available fault injection capabilities}
The Linux fault injection contains many capabilities, each targeting different injection aspects. Following is the list of the fault injection capabilities \cite{LFI_doc}:

\begin{itemize}
    \item \textbf{failslab}:
    Injects slab allocation failures in the Kernel memory allocation functions, such as kmalloc() and kmem\_cache\_alloc(). Slab allocation is a memory management mechanism designed by Sun Micro-systems and introduced in Solaris 5.4. Later on, Unix, like operating systems like FreeBSD and Linux, adapt slabs in their kernels. The Slabs aim to effectively manage the memory allocation of the kernel objects and avoid the memory fragmentation caused by allocating and de-allocating by keeping the caches of commonly used objects in an initialized state available \cite{Slab}.

    \item \textbf{fail\_page\_alloc}:
    Injecting failures in memory pages when allocation. This injection can affect all the functions related to memory page allocation, such as alloc\_pages(), get\_fee\_pages(), etc.
    
    \item \textbf{fail\_usercopy}:
    Injecting failures in user memory access functions like copy\_from\_user(), get\_user(), etc. For example, copy\_from\_user() is a function to copy a block of data from user space; with less checking, this function calls should\_fail\_usercopy() first; if LFI is enabled and debugfs is configured to inject user copy, then the function will fail.
    
    \item \textbf{fail\_futex}:
    Injecting failures in the futex deadlock and user address. Futex is an optimized user-space locking mechanism. The futex() system call offers a mechanism for pausing execution until a specified condition is satisfied.  It is commonly employed as a blocking mechanism in the context of shared-memory synchronization \cite{futex}. However, uaddr represents the user space address of the currently executing task \cite{uaddr}.

    \item \textbf{fail\_sunrpc}:
    Injects failures in the kernel RPC for both client and server. The linux contains a kernel module for SunRPC under thae network file systems called sunrpc.ko since version 2.6.20 \cite{config_sunrpc}. The Sun Remote Procedure Call Protocol is considered a foundational framework for the implementation of Remote Procedure Call (RPC) in numerous distributed computing systems, particularly inside workstation networks operating on UNIX \cite{sunrpc}.

    \item \textbf{fail\_make\_request}:
    Injects disk I/O failures on devices and partitions specified by the path: /sys/block/[device]/[partition]/make-it-fail.

    This failure impacts the submit\_bio\_noacct() kernel function within the block device core, designed to re-submit a bio to the block device layer for input/output operations. The bio defines the position in memory and on the device. \cite{submit_bio}

    When LFI is enabled, and debugfs is configured, the submit\_bio\_noacct() function will call should\_fail\_bio(bio) and then terminate the IO command with the provided status from debugfs.

    \item \textbf{fail\_mmc\_request}:
    Injects MMC data errors on I/O devices under the path /sys/kernel/debug/mmc0/fail\_mmc\_request.

    When MMC starts the request by calling the \_\_mmc\_start\_request() function in the core MMC module in the kernel, the internal function called mmc\_should\_fail\_request() Inject random data errors to the request.

    \item \textbf{fail\_function}:
    Injects error return on specific functions, marked by ALLOW\_ERROR\_INJECTION() macro, by setting debugfs entries under /sys/kernel/debug/fail\_function. This fail capability does not support the boot option.

    For example, to inject ERRNO (a pre-processor macro used for error indication) in the Slab function, we declare the following line in kernel path mm/failslab.c. ALLOW\_ERROR\_INJECTION(should\_failslab, ERRNO);
    %todo add more details from LFI_doc

    \item \textbf{fail\_skb\_realloc}:
    Inject socket buffer (SKB) reallocation events into the network path to detect and prevent problems associated with pointer mishandling in the network subsystem. This feature generates situations where current pointers to SKB headers become invalid by compelling SKB reallocation at crucial locations.
    
    This intentional invalidation reveals code pathways where appropriate pointer update is overlooked following a reallocation event.
    
    By generating these controlled fault situations, the system may identify occurrences of stale pointers, which may result in memory corruption or system instability.

    The following path is utilized to set up the network interface, where devname is the network device name (e.g eth0) /sys/kernel/debug/fail\_skb\_realloc/devname. 
    
    The efficacy of this fault detection is augmented with KASAN enabled since it assists in identifying invalid memory accesses and use-after-free (UAF) problems. 
    
    \item \textbf{NVMe fault injection}:
    Inject NVMe status codes and retry flags on the target devices at the debugfs path: /sys/kernel/debug/nvme*/fault\_inject. The default status code is (NVME\_SC\_INVALID\_OPCODE), without retry. This injection will be discussed in depth in section \ref{section:case_study}. 
    
    \item \textbf{Null test block driver fault injection}:
    This fault injection capability addresses the null block device driver. The null block device (/dev/nullb*) is used to benchmark block-layer implementations. It simulates a block device with a capacity of X gigabytes. It does not perform any actual read or write operations; instead, it marks them as complete in the request queue \cite{null_blk}.

    This category includes the following three faults:
    \begin{enumerate}
        \item Inject IO timeouts by configuring parameters located at: /sys/kernel/config/nullb/[disk]/timeout\_inject

        \item Inject requeue requests by configuring items located at /sys/kernel/config/nullb/[disk]/requeue\_inject

        \item Inject init\_hctx() errors by configuring items located at /sys/kernel/config/nullb/[disk]/init\_hctx\_fault\_inject

    \end{enumerate}

\end{itemize}


\subsubsection{Configure fault-injection capabilities behavior}
There are two methods to configure the LFI capabilities: at boot-time and at runtime configurations. The boot-time configuration of fault capabilities is considered static as you need to reboot the kernel to apply new faults, which makes it suitable for specific faults. On the other hand, the runtime configuration of fault injection compatibilities through debugfs is more flexible as changing the fault and its configuration is done without requiring rebooting \cite{LFI_doc, Naughton}

\begin{enumerate}
    \item \textbf{Runtime configuration}: 
    The fault-inject-debugfs kernel module provides certain debugfs entries for the runtime fault-injection capabilities. Table \ref{tab:Debugfs_Entries1} shows selected entries.

    \begin{table}[ht!]
    \begin{tabular}{|p{0.25\textwidth}|p{0.10\textwidth}|p{0.20\textwidth}|p{0.45\textwidth}|}
    \hline
    \textbf{Debugfs Entry} & \textbf{Input Format} & \textbf{Possible values} & \textbf{Description} \\ \hline
    
    probability & integer & [0,100] & Probability of failed injection. It is important to recognize that a one-failure-per-hundred error rate is excessive for some test scenarios. Set the probability to 100 and configure /sys/kernel/debug/fail*/interval for these test cases. \\ \hline

    interval & long & [0,MAX] & Defines the duration between failures for calls of should\_fail() that successfully meet all other criteria. If interval>1, it is advisable to set probability=100. \\ \hline

    times & integer & [-MAX,MAX] & indicates the maximum allowed occurrences of failures. A value of -1 means "no limit." \\ \hline

    fail*/space &  integer & [-MAX,MAX] & Defines an initial resource "budget," reduced by "size" with each call of should\_fail(, size). Failure injection is blocked until "space" is consumed. \\ \hline

    verbose & integer & {0,1,2} & determines the level of detail in the messages when a fault occurs. ‘0’ indicates no messages; ‘1’ will output a single log entry per failure; ‘2’ will additionally display a call trace, which is beneficial for diagnosing issues exposed by fault injection. \\ \hline

    task-filter & bool &\{Y,N\} & A value of 'N' deactivates process filtering (default setting). Any positive value restricts failures to only those processes specified by /proc/<pid>/make-it-fail==1. \\ \hline


    require-start & long & [0,MAX) & defines the range of virtual addresses evaluated during stack trace traversal. Failure occurs only if a caller in the traversed stack trace falls within the specified range, and none fall within the excluded range. \\ \cline{1-3}
    require-end & long & [0,MAX) &  \\ \cline{1-3}
    reject-start & long & [0,0) &  \\ \cline{1-3}
    reject-end  & long & [0,0) &  \\ \hline

    stacktrace-depth & long & [require-start,require-end), [reject-start,reject-end) & indicates the maximum depth of the stack trace traversed while searching for a caller within the specified range \\ \hline
   
    \end{tabular}
    \caption{Debugfs Entries for failure injection (/sys/kernel/debug/fail*/)}
    \label{tab:Debugfs_Entries1}
    \end{table}    
 
    
    There are two ways to inject the faults during runtime:
    \begin{itemize}
        \item \textbf{debugfs entries}:
        Debugfs is a straightforward mechanism for kernel engineers to expose information to user space. In contrast to /proc, which is exclusively designed for process information, and sysfs, which is strict one-value-per-file rules, debugfs operates without any constraints. Developers may provide any information they desire in that location. The debugfs filesystem is not designed to provide a stable ABI for user space; theoretically, no stability limitations are imposed on the files exported inside \cite{debugfs}.

        To inject faults using debugfs, we write values into specific locations using echo. For example, to force skb reallocation on the network device 'eth0', 1 is assigned to fail\_skb\_realloc path as shown in example \ref{lst:debugfs-echo-example}. It is worth noting that assigning values to debugfs is done with the root permissions.

        \begin{figure}[ht!]
            \centering
            \includegraphics[scale=1]{LFI/debugfs-echo-example.PNG}
            \caption{Force skb reallocation on eth0 \cite{LFI_doc}}
            \label{lst:debugfs-echo-example}
        \end{figure}

        The Linux kernel source code has a script called "failcmd.sh." It is designed to make accomplishing the slab and page allocation failures easier using bash script instead of manually injecting values to debugfs. The script is in the path tools/testing/fault-injection/failed.sh. Example \ref{lst:failcmd_sh_example} shows how to use the script to specify 100 failures at most to inject slab allocation failure.

        \begin{figure}[ht!]
            \centering
            \includegraphics[scale=1]{LFI/failcmd_sh_example.PNG}
            \caption{Inject slab allocation failure using failcmd.sh \cite{LFI_doc}}
            \label{lst:failcmd_sh_example}
        \end{figure}

        \item \textbf{Proc entries}:
        Write and read the integer N to specific file descriptors (/proc//fail-nth, /proc/self/task//fail-nth) to enable all fault types (slab, futex, etc.). This configuration overrides all other generic debugfs options such as probability, interval, times, etc. However, per-capability configurations (e.g., fail\_futex/ignore-private) take precedence over it.

        Writing the integer N to the file descriptors will cause the $N^{th}$ call in the task to fail. The reading from the preceding files yields an integer value. A value of '0' signifies that the fault configuration from a prior writing to this file was introduced. A positive number N signifies that the defect has not yet been injected. 

        This functionality is designed for systematic testing of errors within a singular system call, where developers write a c code to automate the fault injection. For instance, the code in listing \ref{lst:fail-nth-example} systematically faults the $0^{th}, 1^{st}, 2^{nd}, ..., N $, capabilities in the socketpair() system function.  

        \begin{figure}[ht!]
            \centering
            \fcolorbox{black}{white}{
            \includegraphics[scale=.8]{LFI/fail-nth_example.png}
            }
            \caption{Example of fail-nth testing program \cite{LFI_doc}}
            \label{lst:fail-nth-example}
        \end{figure}
        
    \end{itemize}


    \item \textbf{Boot-time}:
    This option is suitable for injecting errors in the early stages of booting when the debugfs are unavailable. In this case, the target fault injection must be assigned in the Linux options line.

\end{enumerate}


\subsubsection{Limitation of Linux fault injection framework}
Despite the LFI being a good starting point to inject fault to target modules with hardware fault type, its time cost is considered medium compared to other tools outside the kernel source, such as LTP \cite{LPT}, KERDR \cite{KERDR}, and others. On the other hand, LFI failed to automate the fault recovery. Due to its design, LFI provides limited experience in injecting failures as it requires considerable effort in complex scenarios. Also, It cannot inject Fault to simulate the device timeouts. Moreover, Faults are injected with a black box approach, with random timing, making tracking the systems logging difficult.

\subsection{Error Injectable Functions}
This section is intended for kernel developers and demonstrates adding a function to the ALLOW\_ERROR\_INJECTION() macro. The function-level error injection alters the code path and produces an error despite appropriate input and conditions. If applied to a non-error-injectable function, it may lead to an unforeseen kernel crash. To add injectable functions, the following requirements must be met \cite{LFI_doc}:
\begin{enumerate}
    \item The function returns an error code upon failure, requiring that the callers verify it correctly. This requirement applies to the functions for releasing objects. A memory leak will rapidly occur if errors in such release functions are not correctly managed. The caller will be confused if the object has been released or corrupted.

    \item The function does not run any code that can alter any state prior to the initial error return. The state includes global, local, or input variables. For instance, clear output address storage (e.g., *ret = NULL), increments/decrements counter, set a flag, preempt/irq disable, or get a lock. This requirement relates to the caller, who anticipates that the function will consistently perform an action. Consequently, if the function error injection bypasses the entire function, the expectation is violated, resulting in an unforeseen error.
\end{enumerate}

Every error-injectable function will possess the error type specified by the ALLOW\_ERROR\_INJECTION() macro. The choice of error type must be made with caution. Introducing a new error-injectable function with an incorrect error type may result in a kernel crash due to inadequate error handling. Four types of errors are listed in include/asm-generic/error-injection.h, as illustrated in Table \ref{tab:Injectable_Functions_errors_types}. 

\begin{table}[ht!]
\begin{tabular}{|p{0.30\textwidth}|p{0.70\textwidth}|}
\hline
\textbf{Error Type} & \textbf{Description} \\ \hline
EI\_ETYPE\_NULL & Return NULL if the function fails. \\ \hline

EI\_ETYPE\_ERRNO & Return an $-errno$ error code if the function fails. For example $-EINVAL$ if the input is wrong.  \\ \hline

EI\_ETYPE\_ERRNO\_NULL & Return a $-errno$ or NULL upon function failure. This type will be suitable if the function caller verifies the return value using the IS\_ERR\_OR\_NULL() macro. \\ \hline

EI\_ETYPE\_TRUE & Return true ($>0$) if the function fails. \\ \hline

\end{tabular}
\caption{Types of function return errors \cite{error_injection_h}}
\label{tab:Injectable_Functions_errors_types}
\end{table} 


\subsubsection{Add new fault injection capability} \label{section:add_new_LFI}
To include new fault injection functionality into a custom device driver or module lacking such support. A number of steps must be performed in order to new fault injection capability:
\begin{enumerate}
    \item Include the fault injection header file (linux/fault-inject.h) into the module source code.
    \item Specify the characteristics of the fault using DECLARE\_FAULT\_ATTRIBUTE(name). The definition of the default structure of the fault attribute (fault\_attr) can be found in (linux/include/linux/fault-inject.h).

    \item Provide the configuration of fault attributes.
    \item The module could require enabling the fault injection capabilities during boot time; the helper function setup\_fault\_attr(attr, str) is employed for this purpose.
    \item The function fault\_create\_debugfs\_attr(name, parent, attr) is utilized to create debugfs attribute. For example, the functions failslab, fail\_page\_alloc, fail\_usercopy, and fail\_make\_request utilize debugfs entries.
    \item If the fault injection capability is restricted to a single kernel module, including module parameters for configuring the fault properties is preferable.
    \item Add a hook to insert failures. When should\_fail() returns true, the client code should inject a failure using should\_fail(attr, size).
\end{enumerate}

\subsubsection{Examples}
This section covers four examples of how to use the Linux fault injection framework as a black box, where errors are injected into the device drivers or modules, and the results are observed from the kernel logs.

\begin{enumerate}
    \item \textbf{Inject slab allocation failures}
    In this example, a slab allocation failures will be injected into the module init/exit code. Linux modules are ELF programs that can be dynamically added to the kernel. They can be detached from the kernel and eliminated when they are no longer required. Primarily, Linux kernel modules consist of device drivers, pseudo-device drivers like network drivers, or file systems \cite{linux_kernel_book}.

    Kernel modules must have at least two functions: an initialization function (init), which is called when the module is "insmod" into the kernel, and a cleanup (exit) function, which is called just before it is removed "rmmod". Both init and exit functions are exposed using the module\_init and module\_exit, respectively \cite{kernel_modules}.

    The example shown in listing \ref{lst:Inject-slab-allocation-failures-example} written in a bash script to facilitate the testing. The script utilizes the debugfs path /sys/kernel/debug/failslab/ and configure the following fault-injection capabilities:

    \begin{enumerate}
        \item The example starts with limiting the failure by setting the task-filter to 'Y'. So this failure will only related to processes indicated by /proc/<pid>/make-it-fail==1. /proc is a mount point for procfs. /proc/self is a symlink to the /proc/<PID> directory, where <PID> is the Process ID of the process accessing /proc at that very instant. 

        \item probability: Set the the failure probability to 10\%.

        \item interval: Specifies the interval between failures by 100. 

        \item times: infinite failure (times -1). 

        \item space: specifies an initial resource "budget" to zero.

        \item verbose: Print a single log line per failure and a call trace.

        \item ignore-gfp-wait: Ignore injecting the failures into allocations that can sleep (\_\_GFP\_DIRECT\_RECLAIM

    \end{enumerate}

    After configuring the slab fault injection through debugfs, the script will call the init function in the module by using the command (modprobe); since the module is configured with the make-it-fail, the Linux fault injection will call should\_fail() function and let the module fail in the initialization phase. Next, the script will call the module's exit function by calling the command (modprobe -r), which does the same thing and calls should\_fail.

    It is worth mentioning that the script is designed to take several modules for injections (\$\*). Please note that injecting errors in critical modules like file systems can cause severe damage to the data.

    \begin{figure}[ht!]
        \centering
        \fcolorbox{black}{white} {
        \includegraphics[scale=0.80]{LFI/Inject-slab-allocation-failures-example.png}
        }
        \caption{Inject slab allocation failures using make\-it\-fail \cite{LFI_doc}}
        \label{lst:Inject-slab-allocation-failures-example}
    \end{figure}   
    
    %todo show the example results

    
    \item \textbf{Inject page allocation failures}
    The example \ref{lst:Inject-page-allocation-failures-example} introduces page allocation failures for specific modules by limiting the range of virtual addresses for the target module through the fault capabilities: require-start and require-end.

    Linux modules are executables in the ELF format. The ELF file comprises multiple sections. The ".text" section contains executable instructions, whereas the ".data" section comprises initialized data that contributes to the program's memory image, in addition to other sections \cite{elf}.

    The example is presented as a bash script that first gets the starting address of the module from "/sys/module/\$module/sections/.text" and subsequently obtains the end address from "/sys/module/\$module/sections/.data". Due to the inability to determine the exact end address of the module, it is assumed that the data section follows immediately after the code section; thus, the starting address of the data section is considered the end address of the code section. This approach is ineffective if the module has a different section order.

    Establishing the task filter functionality is unnecessary as we specify the start and end module addresses in memory, where it is impossible for two modules to occupy the same memory address. The example ignores Get Free Page (GFP) flags for waiting and high memory. The script established the maximum stack trace depth at 10 while locating the caller. The script used the trap command to assign a probability of zero upon the occurrence of a keyboard interruption (Control-C) (SIGINT) or when the process termination signal (SIGTERM) is activated \cite{trap}. Note that the script will continuously inject errors into the module for 11.5 days (sleep 1000000). 

    \begin{figure}[ht!]
        \centering
        \fcolorbox{black}{white} {
        \includegraphics[scale=1]{LFI/Inject-page-allocation-failures-example.png}
        }
        \caption{Inject page allocation failures using "require" capability \cite{LFI_doc}}
        \label{lst:Inject-page-allocation-failures-example}
    \end{figure}  
    %todo show the example results

    \item \textbf{Inject open\_ctree error while btrfs mount}
    The example \ref{lst:fail function mechanism-example} utilizes the fail function mechanism to inject errors in the open\_ctree function while mounting the btrfs. The example is designed as a bash script and starts by creating an image file (test file.img) with a size of 1001 MB and formatting it with the btrfs file system. The BTRFS filesystem has been made the default filesystem in several well-known Linux versions. It utilizes a copy-on-write mechanism, facilitating efficient snapshots and clones. It employs B-trees as its primary on-disk data structure. The design aims to perform effectively across various use cases and workloads \cite{btrfs}. 

    The scripts then configure the Linux fault injection capabilities as follows:
    \begin{enumerate}
        \item set the target function to fail (open\_ctree) into the path /sys/kernel/debug/fail\_function/inject
        
        \item Set the return value to error number 12 (ENOMEM: Out of memory) to path /sys/kernel/debug/fail\_function/open\_ctree/retval 

        \item Disable the task filter
        \item Set the failure probability to 100\%.
        \item No interval between the failures.
        \item Unlimited number of failures (times = -1).
        \item No space limitation.
        \item Print only a single log line per failure.
        
    \end{enumerate}

    Once the mount is done, the script executes the cleanup phase by assigning an empty string to /sys/kernel/debug/fail\_function/inject to turn off the injection, and execute the losetup command to detach the mounted image.

    \begin{figure}[ht!]
        \centering
        \fcolorbox{black}{white} {
        \includegraphics[scale=1]{LFI/fail function mechanism-example.png}
        }
        \caption{Inject fails to open\_ctree while btrfs mounted \cite{LFI_doc}}
        \label{lst:fail function mechanism-example}
    \end{figure}  
    %todo show the example results

    
    \item \textbf{Inject only skbuff allocation failures}
    The listing \ref{lst:Inject-skbuff-failures-example} shows how to inject skbuff allocation failures by marking the buff head cache as faulty, turning on the cache filter for the slab, and finally setting the fault only one time with 1\% probability. As mentioned earlier, "failcmd.sh" can be used to automate the slab injection.

    \begin{figure}[ht!]
        \centering
        \fcolorbox{black}{white} {
        \includegraphics[scale=1]{LFI/Inject-skbuff-failures-example.png}
        }
        \caption{Inject only skbuff allocation failures \cite{LFI_doc}}
        \label{lst:Inject-skbuff-failures-example}
    \end{figure}
    %todo show the example results

    
\end{enumerate}

\subsubsection{Case study: NVMe Fault Injection} \label{section:case_study}    
This section briefly introduces the NVMe Fault Injection by discussing the NVMe driver internals. By default, the Linux fault injection framework will inject the NVME\_SC\_INVALID\_OPCODE status code with no retry into the nvme\_try\_complete\_req. There are lots of NVMe status values that could be injected into the driver; figure \ref{fig:nvme_cmd_status} shows a set of the generic NVME command status; the complete list can be found in include/linux/nvme.h.

\begin{figure}[ht!]
    \centering
    \fcolorbox{black}{white} {
    \includegraphics[scale=0.90]{LFI/nvme_cmd_status.png}
    }
    \caption{Subset of generic NVMe command Status \cite{nvme_header}}
    \label{fig:nvme_cmd_status}
\end{figure}


The nvme\_try\_complete\_req function is part of the NVMe host driver; the function aims to fill in the status and result in the information from the completion queue entry (CQE). The function is designed to inject status failures from the injection framework by calling the function nvme\_should\_fail, as shown in Figure \ref{fig:nvme_try_complete_req}.

\begin{figure}[ht!]
    \centering
    \fcolorbox{black}{white} {
    \includegraphics[scale=0.80]{LFI/nvme_try_complete_req.png}
    }
    \caption{NVMe nvme\_try\_complete\_req function \cite{host_nvme_header} }
    \label{fig:nvme_try_complete_req}
\end{figure}

The implementation of nvme\_should\_fail is found in the path (linux/drivers/nvme/host/fault\_inject.c). The function injects the status code and DNR bit, as shown in Figure \ref{fig:nvme_should_fail}.

\begin{figure}[ht!]
    \centering
    \fcolorbox{black}{white} {
    \includegraphics[scale=0.80]{LFI/nvme_should_fail.png}
    }
    \caption{NVMe nvme\_try\_complete\_req function \cite{host_nvme_code} }
    \label{fig:nvme_should_fail}
\end{figure}

Example \ref{lst:nvme_inject-example} shows how to inject the default NVMe status code without retrying into nvme0n1 disk. By executing the copy command, the following functions will be called sequentially: nvme\_try\_complete\_req $\rightarrow$ nvme\_should\_fail $\rightarrow$ should\_fail. The expected result is shown in listing \ref{lst:nvme_inject-expected-result}, and the kernel logs (dmesg) are shown in listing \ref{lst:nvme_inject-kernel-message}.

\begin{figure}[ht!]
    \centering
    \fcolorbox{black}{white} {
    \includegraphics[scale=1]{LFI/nvme_inject-example.png}
    }
    \caption{Inject default NVMe status code with no retry example \cite{nvme_fault_inject}}
    \label{lst:nvme_inject-example}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[scale=1]{LFI/nvme_inject-expected-result.PNG}
    \caption{Inject default NVMe status expected result}
    \label{lst:nvme_inject-expected-result}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[scale=1]{LFI/nvme_inject-kernel-message.PNG}
    \caption{NVMe default injection kernel message}
    \label{lst:nvme_inject-kernel-message}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
    
